Monitoring Deforestation Using Multivariate Bayesian Online Changepoint Detection with Outliers

Near real time change detection is important for a variety of Earth monitoring applications and remains a high priority for remote sensing science. Data sparsity, subtle changes, seasonal trends, and the presence of outliers make detecting actual landscape changes challenging. Adams and MacKay (2007) introduced Bayesian Online Changepoint Detection (BOCPD), a computationally efficient, exact Bayesian method for change detection. Incorporation of prior information allows for relaxed dependence on dense data and an extensive stable period, making this method applicable to relatively short time series and multiple changepoint detection. In this paper we conduct BOCPD with a multivariate linear regression framework that supports seasonal trends. We introduce a mechanism to make BOCPD robust against occasional outliers without compromising the computational efficiency of an exact posterior change distribution nor the detection latency. We show via simulations that the method effectively detects change in the presence of outliers. The method is then applied to monitor deforestation in Myanmar where we show superior performance compared to current online changepoint detection methods.

==> MUTATED (2)/commands.tex <==
\newcommand{\btheta}{ \mbox{\boldmath $\theta$}}
\newcommand{\bmu}{ \mbox{\boldmath $\mu$}}
\newcommand{\balpha}{ \mbox{\boldmath $\alpha$}}
\newcommand{\bbeta}{ \mbox{\boldmath $\beta$}}
\newcommand{\bmeta}{ \mbox{\boldmath $\eta$}}
\newcommand{\bdelta}{ \mbox{\boldmath $\delta$}}
\newcommand{\blambda}{ \mbox{\boldmath $\lambda$}}
\newcommand{\bgamma}{ \mbox{\boldmath $\gamma$}}
\newcommand{\brho}{ \mbox{\boldmath $\rho$}}
\newcommand{\bpsi}{ \mbox{\boldmath $\psi$}}
\newcommand{\bepsilon}{ \mbox{\boldmath $\epsilon$}}
\newcommand{\bomega}{ \mbox{\boldmath $\omega$}}
\newcommand{\bDelta}{ \mbox{\boldmath $\Delta$}}
\newcommand{\bSigma}{ \mbox{\boldmath $\Sigma$}}
\newcommand{\bOmega}{ \mbox{\boldmath $\Omega$}}
\newcommand{\bGamma}{ \mbox{\boldmath $\Gamma$}}

\newcommand{\bA}{ \mbox{\bf A}}
\newcommand{\ba}{ \mbox{\bf a}}
\newcommand{\be}{ \mbox{\bf e}}
\newcommand{\bP}{ \mbox{\bf P}}
\newcommand{\bx}{ \mbox{\bf x}}
\newcommand{\bX}{ \mbox{\bf X}}
\newcommand{\bB}{ \mbox{\bf B}}
\newcommand{\bZ}{ \mbox{\bf Z}}
\newcommand{\by}{ \mbox{\bf y}}
\newcommand{\bY}{ \mbox{\bf Y}}
\newcommand{\bz}{ \mbox{\bf z}}
\newcommand{\bh}{ \mbox{\bf h}}
\newcommand{\bmm}{ \mbox{\bf m}}
\newcommand{\br}{ \mbox{\bf r}}
\newcommand{\bt}{ \mbox{\bf t}}
\newcommand{\bs}{ \mbox{\bf s}}
\newcommand{\bb}{ \mbox{\bf b}}
\newcommand{\bff}{ \mbox{\bf f}}
\newcommand{\bL}{ \mbox{\bf L}}
\newcommand{\bu}{ \mbox{\bf u}}
\newcommand{\bv}{ \mbox{\bf v}}
\newcommand{\bV}{ \mbox{\bf V}}
\newcommand{\bG}{ \mbox{\bf G}}
\newcommand{\bC}{ \mbox{\bf C}}
\newcommand{\bg}{ \mbox{\bf g}}
\newcommand{\bH}{ \mbox{\bf H}}
\newcommand{\bI}{ \mbox{\bf I}}
\newcommand{\bD}{ \mbox{\bf D}}
\newcommand{\bM}{ \mbox{\bf M}}
\newcommand{\bW}{ \mbox{\bf W}}
\newcommand{\bw}{ \mbox{\bf w}}
\newcommand{\bT}{ \mbox{\bf T}}
\newcommand{\bQ}{ \mbox{\bf Q}}
\newcommand{\bR}{ \mbox{\bf R}}
\newcommand{\bfe}{ \mbox{\bf e}}
\newcommand{\bzero}{ \mbox{\bf 0}}

\newcommand{\iid}{\stackrel{iid}{\sim}}
\newcommand{\indep}{\stackrel{indep}{\sim}}
\newcommand{\Xtil}{{\tilde X}}
\newcommand{\bXtil}{\bf {\tilde X}}

\newcommand{\calR}{{\cal R}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calA}{{\cal A}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calK}{{\cal K}}

\newcommand{\argmax}{{\mathop{\rm arg\, max}}}
\newcommand{\argmin}{{\mathop{\rm arg\, min}}}
\newcommand{\Frechet}{\mbox{Fr$\acute{\mbox{e}}$chet}}
\newcommand{\Matern}{ \mbox{Mat$\acute{\mbox{e}}$rn}}
\newcommand{\Prob}{\mbox{Prob}}

\newcommand{\beq}{ \begin{equation}}
\newcommand{\eeq}{ \end{equation}}
\newcommand{\beqn}{ \begin{eqnarray}}
\newcommand{\eeqn}{ \end{eqnarray}}



==> MUTATED (2)/tabs/myanmar_results_table.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Wed Dec 22 23:21:43 2021
\begin{table}[H]
\centering
\caption{Summary statistics for detection of the first change point in annotated Myanmar deforestation data.} 
\label{tab:myanmar_results}
\begin{tabular}{rlllll}
  \hline
 Metric & TP & FP & F-score & Latency & Time (ms) \\ 
   \hline
CCD & 0.85 & 0.45 & 0.88 & 2.00 & 3.98 \\ 
  BOCPDMS & 0.34 & 0.89 & 0.67 & 3.00 & 32.54 \\ 
  rBOCPDMS & 0.02 & 0.06 & 0.66 & 25.00 & 1110.64 \\ 
  BOCPD & 0.95 & 0.65 & 0.88 & 3.32 & 5.44 \\ 
  BOCPD-OD & 0.87 & 0.32 & 0.90 & 2.27 & 30.50 \\ 
  \end{tabular}
\end{table}


==> MUTATED (2)/tabs/myanmar_results_table_outliers.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Wed Dec 08 09:57:42 2021
\begin{table}[ht]
\centering
\begin{tabular}{rlllll}
  \hline
 Metric & \lvert TP \rvert & \lvert FP \rvert & F-score & Latency & Time (s) \\ 
   \hline
CCD & 0.85 & 0.45 & 0.88 & 2.00 & 0.16 \\ 
  BOCPDMS & 0.63 & 1.07 & 0.72 & 1.85 & 1.30 \\ 
  rBOCPDMS & 0.02 & 0.04 & 0.67 & 23.00 & 32.90 \\ 
  BOCPD & 0.95 & 0.67 & 0.82 & 3.30 & 0.22 \\ 
  BOCPD-OD & 0.93 & 0.45 & 0.85 & 2.29 & 1.37 \\ 
  \end{tabular}
\caption{Summary statistics for detection of the first change point in annotated Myanmar deforestation data.} 
\end{table}


==> MUTATED (2)/tabs/myanmar_sensitivity_results_table.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Wed Dec 22 23:22:47 2021
\begin{table}[H]
\centering
\caption{Summary statistics comparing sensitivity of BOCPD-OD to priors and tuning parameters of detection of the first change point in annotated Myanmar deforestation data.} 
\label{tab:myanmar_sensitivity_results}
\begin{tabular}{lllllllllll}
  \hline
$\Lambda_0$ scale & $\nu_0$ & $\alpha$ & $p_o$ & $V_0$ scale & L & TP & FP & F-score & Latency & Time (ms) \\ 
  \hline
1 &  4.82 & 0.9 & 0.5 & 1 & 3 & 0.74 & 0.32 & 0.86 & 2.46 & 27.15 \\ 
  10 &  4.82 & 0.9 & 0.5 & 1 & 3 & 0.72 & 0.33 & 0.85 & 2.32 & 27.23 \\ 
  0.1 &  4.82 & 0.9 & 0.5 & 1 & 3 & 0.76 & 0.39 & 0.86 & 2.33 & 29.19 \\ 
  0.01 &  4.82 & 0.9 & 0.5 & 1 & 3 & 0.74 & 0.46 & 0.85 & 2.21 & 29.12 \\ 
  1 &  3.01 & 0.9 & 0.5 & 1 & 3 & 0.68 & 0.43 & 0.83 & 2.54 & 27.86 \\ 
  1 & 10.00 & 0.9 & 0.5 & 1 & 3 & 0.73 & 0.29 & 0.86 & 2.33 & 29.79 \\ 
  1 &  4.82 & 0.5 & 0.5 & 1 & 3 & 0.68 & 0.25 & 0.85 & 2.67 & 23.26 \\ 
  1 &  4.82 & 0.9 & 0.1 & 1 & 3 & 0.73 & 0.29 & 0.86 & 2.49 & 28.63 \\ 
  1 &  4.82 & 0.9 & 0.9 & 1 & 3 & 0.75 & 0.38 & 0.85 & 2.33 & 31.63 \\ 
  1 &  4.82 & 0.9 & 0.5 & 0.1 & 3 & 0.75 & 0.43 & 0.85 & 2.56 & 29.65 \\ 
  1 &  4.82 & 0.9 & 0.5 & 10 & 3 & 0.63 & 0.27 & 0.83 & 2.10 & 29.21 \\ 
  1 &  4.82 & 0.9 & 0.5 & 1 & 5 & 0.76 & 0.33 & 0.87 & 2.46 & 30.55 \\ 
  1 &  4.82 & 0.9 & 0.5 & 1 & 1 & 0.65 & 0.26 & 0.84 & 2.58 & 21.54 \\ 
  \end{tabular}
\end{table}


==> MUTATED (2)/tabs/ss_metrics_table.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Wed Dec 22 23:51:28 2021
\begin{table}[H]
\centering
\caption{Average metrics (standard errors are in subscripts) for the simulation
study. The scenarios are defined in Table 1.\\} 
\label{tab:sim_results}
\begin{tabular}{rllllll}
  \hline
Scenario & Method & TP & FP & F-score & Latency & Time (ms) \\ 
  \hline
  1 & CCD & 0.76\textsubscript{4e-04} & 0.34\textsubscript{5e-04} & 0.86\textsubscript{2e-04} & 2.00\textsubscript{0.00} & 6.26\textsubscript{7e-04} \\ 
    1 & BOCPDMS & 1.00\textsubscript{3e-05} & 1.06\textsubscript{0.001} & 0.82\textsubscript{2e-04} & 2.90\textsubscript{0.001} & 17.74\textsubscript{2e-04} \\ 
    1 & rBOCPDMS & 0.99\textsubscript{0.001} & 0.20\textsubscript{0.006} & 0.96\textsubscript{0.001} & 21.19\textsubscript{0.05} & 2709.05\textsubscript{2.31} \\ 
    1 & BOCPD & 0.94\textsubscript{2e-04} & 1.03\textsubscript{5e-04} & 0.79\textsubscript{1e-04} & 3.47\textsubscript{0.002} & 24.62\textsubscript{0.001} \\ 
    1 & BOCPD-OD & 0.99\textsubscript{1e-04} & 0.32\textsubscript{6e-04} & 0.94\textsubscript{1e-04} & 3.34\textsubscript{8e-04} & 30.00\textsubscript{0.002} \\ 
   \hline
  2 & CCD & 1.00\textsubscript{0.00} & 0.11\textsubscript{3e-04} & 0.98\textsubscript{6e-05} & 2.00\textsubscript{0.00} & 6.22\textsubscript{7e-04} \\ 
    2 & BOCPDMS & 1.00\textsubscript{0.00} & 1.29\textsubscript{0.001} & 0.79\textsubscript{2e-04} & 1.27\textsubscript{0.001} & 17.76\textsubscript{1e-04} \\ 
    2 & rBOCPDMS & 0.94\textsubscript{0.002} & 0.28\textsubscript{0.006} & 0.93\textsubscript{0.001} & 33.57\textsubscript{0.10} & 2713.88\textsubscript{1.97} \\ 
    2 & BOCPD & 1.00\textsubscript{3e-05} & 1.02\textsubscript{4e-04} & 0.80\textsubscript{7e-05} & 3.40\textsubscript{0.002} & 24.36\textsubscript{0.001} \\ 
    2 & BOCPD-OD & 1.00\textsubscript{0.00} & 0.29\textsubscript{6e-04} & 0.95\textsubscript{1e-04} & 3.29\textsubscript{0.001} & 30.14\textsubscript{0.002} \\ 
   \hline
  3 & CCD & 0.66\textsubscript{5e-04} & 0.49\textsubscript{6e-04} & 0.81\textsubscript{2e-04} & 2.00\textsubscript{0.00} & 6.27\textsubscript{7e-04} \\ 
    3 & BOCPDMS & 1.00\textsubscript{0.00} & 1.62\textsubscript{0.001} & 0.75\textsubscript{2e-04} & 2.62\textsubscript{0.002} & 17.84\textsubscript{3e-04} \\ 
    3 & rBOCPDMS & 0.98\textsubscript{0.001} & 0.37\textsubscript{0.008} & 0.93\textsubscript{0.001} & 19.68\textsubscript{0.06} & 2796.65\textsubscript{2.23} \\ 
    3 & BOCPD & 0.92\textsubscript{3e-04} & 0.91\textsubscript{3e-04} & 0.80\textsubscript{1e-04} & 3.64\textsubscript{0.002} & 24.61\textsubscript{0.002} \\ 
    3 & BOCPD-OD & 0.99\textsubscript{1e-04} & 0.04\textsubscript{2e-04} & 0.99\textsubscript{6e-05} & 3.65\textsubscript{0.002} & 30.09\textsubscript{0.002} \\ 
   \hline
  4 & CCD & 1.00\textsubscript{5e-05} & 0.16\textsubscript{4e-04} & 0.97\textsubscript{8e-05} & 2.00\textsubscript{0.00} & 6.41\textsubscript{7e-04} \\ 
    4 & BOCPDMS & 1.00\textsubscript{3e-05} & 1.76\textsubscript{0.001} & 0.73\textsubscript{2e-04} & 1.41\textsubscript{0.001} & 17.91\textsubscript{1e-04} \\ 
    4 & rBOCPDMS & 0.88\textsubscript{0.003} & 0.50\textsubscript{0.007} & 0.87\textsubscript{0.002} & 33.82\textsubscript{0.10} & 2925.90\textsubscript{2.10} \\ 
    4 & BOCPD & 1.00\textsubscript{4e-05} & 0.93\textsubscript{3e-04} & 0.81\textsubscript{5e-05} & 3.31\textsubscript{0.002} & 26.19\textsubscript{0.002} \\ 
    4 & BOCPD-OD & 1.00\textsubscript{0.00} & 0.02\textsubscript{1e-04} & 1.00\textsubscript{3e-05} & 3.09\textsubscript{6e-04} & 30.16\textsubscript{0.002} \\ 
   \hline
  5 & CCD & 0.77\textsubscript{4e-04} & 0.35\textsubscript{5e-04} & 0.86\textsubscript{2e-04} & 2.00\textsubscript{0.00} & 7.00\textsubscript{0.001} \\ 
    5 & BOCPD & 0.97\textsubscript{2e-04} & 0.92\textsubscript{3e-04} & 0.81\textsubscript{8e-05} & 3.41\textsubscript{0.002} & 26.48\textsubscript{0.002} \\ 
    5 & BOCPD-OD & 0.99\textsubscript{1e-04} & 0.18\textsubscript{4e-04} & 0.96\textsubscript{9e-05} & 3.17\textsubscript{0.001} & 32.23\textsubscript{0.002} \\ 
   \hline
  6 & CCD & 0.99\textsubscript{8e-05} & 0.12\textsubscript{3e-04} & 0.97\textsubscript{8e-05} & 2.00\textsubscript{0.00} & 7.06\textsubscript{0.001} \\ 
    6 & BOCPD & 1.00\textsubscript{0.00} & 0.92\textsubscript{3e-04} & 0.82\textsubscript{6e-05} & 3.14\textsubscript{0.001} & 26.27\textsubscript{0.002} \\ 
    6 & BOCPD-OD & 1.00\textsubscript{0.00} & 0.15\textsubscript{4e-04} & 0.97\textsubscript{7e-05} & 3.06\textsubscript{6e-04} & 32.34\textsubscript{0.002} \\ 
   \hline
  7 & CCD & 0.72\textsubscript{5e-04} & 0.45\textsubscript{6e-04} & 0.83\textsubscript{2e-04} & 2.00\textsubscript{0.00} & 6.83\textsubscript{0.001} \\ 
    7 & BOCPD & 0.87\textsubscript{3e-04} & 0.91\textsubscript{3e-04} & 0.78\textsubscript{1e-04} & 3.80\textsubscript{0.003} & 26.62\textsubscript{0.002} \\ 
    7 & BOCPD-OD & 0.95\textsubscript{2e-04} & 0.03\textsubscript{2e-04} & 0.98\textsubscript{9e-05} & 3.60\textsubscript{0.002} & 32.16\textsubscript{0.003} \\ 
   \hline
  8 & CCD & 0.98\textsubscript{1e-04} & 0.20\textsubscript{4e-04} & 0.96\textsubscript{1e-04} & 2.00\textsubscript{0.00} & 6.88\textsubscript{0.001} \\ 
    8 & BOCPD & 0.99\textsubscript{1e-04} & 0.93\textsubscript{3e-04} & 0.81\textsubscript{6e-05} & 3.38\textsubscript{0.002} & 27.83\textsubscript{0.003} \\ 
    8 & BOCPD-OD & 1.00\textsubscript{5e-05} & 0.02\textsubscript{2e-04} & 1.00\textsubscript{3e-05} & 3.07\textsubscript{5e-04} & 32.49\textsubscript{0.002} \\ 
   \hline
  9 & CCD & 0.10\textsubscript{3e-04} & 0.93\textsubscript{3e-04} & 0.55\textsubscript{1e-04} & 2.00\textsubscript{0.00} & 5.90\textsubscript{5e-04} \\ 
    9 & BOCPD & 0.68\textsubscript{5e-04} & 0.91\textsubscript{3e-04} & 0.72\textsubscript{2e-04} & 5.58\textsubscript{0.004} & 24.08\textsubscript{0.001} \\ 
    9 & BOCPD-OD & 0.81\textsubscript{4e-04} & 0.13\textsubscript{3e-04} & 0.91\textsubscript{2e-04} & 5.31\textsubscript{0.004} & 27.71\textsubscript{0.002} \\ 
   \hline
\end{tabular}
\end{table}


==> MUTATED (2)/tabs/ss_sensitivity_metrics_table.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Thu Dec 23 00:28:12 2021
\begin{table}[H]
\centering
\caption{Average metrics (standard errors are in subscripts) for the simulation sensitivity
study applied to scenario 7.\\} 
\label{tab:sim_sensitivity_results}
\begin{tabular}{lllllllllll}
  \hline
$\mu$ & $\Lambda_0$ scale & $\nu_0$ & $\alpha$ & $p_o$ & L & TP & FP & F-score & Latency & Time (ms) \\ 
  \hline
0.5 & 1 & 20 & 0.9 & 0.5 & 5 & 0.92\textsubscript{3e-04} & 0.04\textsubscript{2e-04} & 0.97\textsubscript{1e-04} & 3.87\textsubscript{0.002} & 30.25\textsubscript{0.002} \\ 
  0.4 & 1 & 20 & 0.9 & 0.5 & 5 & 0.92\textsubscript{3e-04} & 0.03\textsubscript{2e-04} & 0.97\textsubscript{1e-04} & 3.93\textsubscript{0.003} & 30.29\textsubscript{0.002} \\ 
  0.5 & 0.01 & 20 & 0.9 & 0.5 & 5 & 0.86\textsubscript{3e-04} & 0.02\textsubscript{2e-04} & 0.95\textsubscript{1e-04} & 4.41\textsubscript{0.003} & 30.02\textsubscript{0.002} \\ 
  0.5 & 100 & 20 & 0.9 & 0.5 & 5 & 0.83\textsubscript{4e-04} & 0.07\textsubscript{3e-04} & 0.93\textsubscript{1e-04} & 5.21\textsubscript{0.004} & 29.70\textsubscript{0.002} \\ 
  0.5 & 1 & 4 & 0.9 & 0.5 & 5 & 0.95\textsubscript{2e-04} & 0.06\textsubscript{3e-04} & 0.97\textsubscript{9e-05} & 3.98\textsubscript{0.003} & 30.73\textsubscript{0.002} \\ 
  0.5 & 1 & 50 & 0.9 & 0.5 & 5 & 0.91\textsubscript{3e-04} & 0.04\textsubscript{2e-04} & 0.96\textsubscript{1e-04} & 3.91\textsubscript{0.002} & 30.58\textsubscript{0.002} \\ 
  0.5 & 1 & 20 & 0.5 & 0.5 & 5 & 0.93\textsubscript{3e-04} & 0.02\textsubscript{1e-04} & 0.97\textsubscript{1e-04} & 4.30\textsubscript{0.003} & 30.59\textsubscript{0.002} \\ 
  0.5 & 1 & 20 & 0.9 & 0.1 & 5 & 0.91\textsubscript{3e-04} & 0.02\textsubscript{2e-04} & 0.97\textsubscript{1e-04} & 4.14\textsubscript{0.003} & 30.67\textsubscript{0.002} \\ 
  0.5 & 1 & 20 & 0.9 & 0.9 & 5 & 0.92\textsubscript{3e-04} & 0.07\textsubscript{3e-04} & 0.96\textsubscript{1e-04} & 3.79\textsubscript{0.002} & 30.92\textsubscript{0.002} \\ 
  0.5 & 1 & 20 & 0.9 & 0.5 & 1 & 0.74\textsubscript{4e-04} & 0.01\textsubscript{1e-04} & 0.91\textsubscript{1e-04} & 3.91\textsubscript{0.003} & 30.64\textsubscript{0.002} \\ 
  0.5 & 1 & 20 & 0.9 & 0.5 & 3 & 0.89\textsubscript{3e-04} & 0.03\textsubscript{2e-04} & 0.96\textsubscript{1e-04} & 3.94\textsubscript{0.003} & 30.93\textsubscript{0.002} \\ 
  \end{tabular}
\end{table}


==> tabs/myanmar_results_table_outliers.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Wed Dec 08 09:57:42 2021
\begin{table}[ht]
\centering
\begin{tabular}{rlllll}
  \hline
 Metric & \lvert TP \rvert & \lvert FP \rvert & F-score & Latency & Time (s) \\ 
   \hline
CCD & 0.85 & 0.45 & 0.88 & 2.00 & 0.16 \\ 
  BOCPDMS & 0.63 & 1.07 & 0.72 & 1.85 & 1.30 \\ 
  rBOCPDMS & 0.02 & 0.04 & 0.67 & 23.00 & 32.90 \\ 
  BOCPD & 0.95 & 0.67 & 0.82 & 3.30 & 0.22 \\ 
  BOCPD-OD & 0.93 & 0.45 & 0.85 & 2.29 & 1.37 \\ 
  \end{tabular}
\caption{Summary statistics for detection of the first change point in annotated Myanmar deforestation data.} 
\end{table}

